FL-DECO-BC: A Privacy-Preserving, Provably Secure, and Provenance-Preserving Federated Learning Framework with Decentralized Oracles on Blockchain for VANETs

Vehicular Ad-Hoc Networks (VANETs) hold immense potential for improving traffic safety and efficiency. However, traditional centralized approaches for machine learning in VANETs raise concerns about data privacy and security. Federated Learning (FL) offers a solution that enables collaborative model training without sharing raw data. This paper proposes FL-DECO-BC as a novel privacy-preserving, provably secure, and provenance-preserving federated learning framework specifically designed for VANETs. FL-DECO-BC leverages decentralized oracles on blockchain to securely access external data sources while ensuring data privacy through advanced techniques. The framework guarantees provable security through cryptographic primitives and formal verification methods. Furthermore, FL-DECO-BC incorporates a provenance-preserving design to track data origin and history, fostering trust and accountability. This combination of features empowers VANETs with secure and privacy-conscious machine-learning capabilities, paving the way for advanced traffic management and safety applications.

==> name.tex <==
\begin{thebibliography}{00}
\bibitem{b1} M. A. Al-Shareeda, M. Anbar, S. Manickam, A. Khalil and I. H. Hasbullah, ``Security and Privacy Schemes in Vehicular Ad-Hoc Network With Identity-Based Cryptography Approach: A Survey`, in IEEE Access, vol. 9, pp. 121522-121531, 2021, doi: 10.1109/ACCESS.2021.3109264

\bibitem{b2} Elsagheer, Samir \& AlShalfan, Khaled. (2021). Intelligent Traffic Management System Based on the Internet of Vehicles (IoV). \textit{Journal of Advanced Transportation}, 1-23. doi:10.1155/2021/4037533.

\bibitem{b3} Arya, M.; Sastry, H.; Dewangan, B.K.; Rahmani, M.K.I.; Bhatia, S.; Muzaffar, A.W.; Bivi, M.A. Intruder Detection in VANET Data Streams Using Federated Learning for Smart City Environments. Electronics 2023, 12, 894. https://doi.org/10.3390/electronics12040894
\bibitem{b4} Rehman, Sabih \& Khan, M. Arif \& Zia, Tanveer \& Zheng, Lihong. (2013). Vehicular ad-hoc networks (VANETs)—An overview and challenges. \textit{Journal of Wireless Networking and Communications}, 3, 29-38. doi:10.5923/j.jwnc.20130303.02.

\bibitem{b5} Ziyao Liu, Jiale Guo, Wenzhuo Yang, Jiani Fan, Kwok-Yan Lam, and Jun Zhao.``Privacy-Preserving Aggregation in Federated Learning: A Survey.` arXiv preprint arXiv:2203.17005 (2022). [Online]. Available: https://arxiv.org/abs/2203.17005

\bibitem{b6} Abdeljalil Beniiche.``A Study of Blockchain Oracles.` arXiv preprint arXiv:2004.07140 (2020). [Online]. Available: https://arxiv.org/abs/2004.07140

\bibitem{b7} L. Gigli, I. Zyrianoff, F. Montori, C. Aguzzi, L. Roffia and M. Di Felice, ``A Decentralized Oracle Architecture for a Blockchain-Based IoT Global Market,` in IEEE Communications Magazine, vol. 61, no. 8, pp. 86-92, August 2023, doi: 10.1109/MCOM.007.2200906. 
\bibitem{b8} McMahan, B., Moore, E., Ramage, D., Hampson, S. and y Arcas, B.A., 2017, April. Communication-efficient learning of deep networks from decentralized data. In Artificial intelligence and statistics (pp. 1273-1282). PMLR.



\bibitem{b9} S. Suo, K. Huang, X. Kuang, Y. Cao, L. Chen and W. Tao, ``Implementation of Low Delay Distribution Terminal Security Protection,` 2021 IEEE International Conference on Consumer Electronics and Computer Engineering (ICCECE), Guangzhou, China, 2021, pp. 140-143, doi: 10.1109/ICCECE51280.2021.9342232.

\bibitem{b10} Xu, M., Chen, X. \& Kou, G. A systematic review of blockchain. Financ Innov 5, 27 (2019). https://doi.org/10.1186/s40854-019-0147-z
\bibitem{b11}Wenhua, Z.; Qamar, F.; Abdali, T.-A.N.; Hassan, R.; Jafri, S.T.A.; Nguyen, Q.N. Blockchain Technology: Security Issues, Healthcare Applications, Challenges and Future Trends. Electronics 2023, 12, 546. https://doi.org/10.3390/electronics12030546



\bibitem{b12}Hasan, Jahid. (2019). Overview and applications of Zero Knowledge Proof (ZKP). 8. 5. 
\bibitem{b13}Chuan Zhao, Shengnan Zhao, Minghao Zhao, Zhenxiang Chen, Chong-Zhi Gao, Hongwei Li, Yu-an Tan,
Secure Multi-Party Computation: Theory, practice and applications,
Information Sciences,
Volume 476,
2019,
Pages 357-372,
ISSN 0020-0255,
https://doi.org/10.1016/j.ins.2018.10.024.
(https://www.sciencedirect.com/science/article/pii/S0020025518308338)
\bibitem{b14} Chainlink 2.0: A Decentralized Oracle Network for Secure Smart Contract Automation //done
\bibitem{b16}Zhang, R., Wang, H., Li, B., Cheng, X., \& Yang, L. (2024). A Survey on Federated Learning in Intelligent Transportation Systems. arXiv preprint arXiv:2403.07444.


\bibitem{b17}Zhang, Y., Chen, Y., Yang, L., Liu, S., \& Cao, J. (2021, June). Federated Learning for Cooperative Traffic Signal Control in VANETs. IEEE: 
https://ieeexplore.ieee.org/abstract/document/9392372


\bibitem{b18}Huang, J., Xu, J., \& Wang, Y. (2020, December). Federated Learning for Green Routing in VANETs. IEEE: https://ieeexplore.ieee.org/document/9084352



\bibitem{b19}Sun, Y., Song, H., Xu, C., \& Li, S. (2022, September). Federated Learning for Collaborative Drowsiness Detection in VANETs. IEEE: https://ieeexplore.ieee.org/document/9833516



\bibitem{b20}Wei, H., Wu, Y., Tang, X., \& Zhou, X. (2021, June). Federated Learning for Joint Vehicle Speed and Traffic Flow Prediction in VANETs. IEEE: https://ieeexplore.ieee.org/document/9950054
\bibitem{b21}Routis, K., Spyropoulos, T., \&  Papadimitriou, V. (2024). A Secure and Privacy Preserved Infrastructure for VANETs based on Federated Learning with Local Differential Privacy. ScienceDirect: https://www.sciencedirect.com/science/article/abs/pii/S0020025523013026
\bibitem{b22}Sierra, José \& Hernandez-Castro, Julio \& Alcaide, Almudena \& Torres, Joaquín. (1970). Validating the use of BAN LOGIC. 3043. 851-858. 10.1007/978-3-540-24707-4\_98. 



\bibitem{b23}Jin, W., Yao, Y., Han, S., Joe-Wong, C., Ravi, S., Avestimehr, S., \& He, C. (2023). FedML-HE: An Efficient Homomorphic-Encryption-Based Privacy-Preserving Federated Learning System. arXiv preprint arXiv:2303.10837.



\bibitem{b24}Sneha Kanchan, Jae Won Jang, Jun Yong Yoon, Bong Jun Choi,Efficient and privacy-preserving group signature for federated learning,Future Generation Computer Systems,Volume 147,2023, Pages 93-106,ISSN 0167-739X,https://doi.org/10.1016/j.future.2023.04.017.
(https://www.sciencedirect.com/science/article/pii/S0167739X23001528).
\bibitem{b25}Chen, Q., You, Z., \& Jiang, H. (2021). Semi-asynchronous Hierarchical Federated Learning for Cooperative Intelligent Transportation Systems. arXiv preprint arXiv:2110.09073.
\bibitem{b26}Song, R., Lyu, L., Jiang, W., Festag, A., \& Knoll, A. (2023). V2X-Boosted Federated Learning for Cooperative Intelligent Transportation Systems with Contextual Client Selection. arXiv preprint arXiv:2305.11654.


\end{thebibliography}
